Mitigating Over-smoothing in Transformers via Regularized Nonlocal Functionals

Transformers have achieved remarkable success in a wide range of natural language processing and computer vision applications. However, the representation capacity of a deep transformer model is degraded due to the over-smoothing issue in which the token representations become identical when the model's depth grows. In this work, we show that self-attention layers in transformers minimize a functional which promotes smoothness, thereby causing token uniformity. We then propose a novel regularizer that penalizes the norm of the difference between the smooth output tokens from self-attention and the input tokens to preserve the fidelity of the tokens. Minimizing the resulting regularized energy functional, we derive the Neural Transformer with a Regularized Nonlocal Functional (NeuTRENO), a novel class of transformer models that can mitigate the over-smoothing issue. We empirically demonstrate the advantages of NeuTRENO over the baseline transformers and state-of-the-art methods in reducing the over-smoothing of token representations on various practical tasks, including object classification, image segmentation, and language modeling.

==> primal_dual_transformer/iclr_2023/method_tan.tex <==
% {\color{red} In image processing, the total variation method~\cite{RUDIN1992259} is commonly used for image denoising.
% A total variation of an image is given by:
% \begin{align}
% \text{TV}(\bv) = \int |\nabla\bv(\bz)| d\bz,
% \end{align}
% where $z = [z_1, z_2]^T \in \Omega^2$ is the position variable. 
% Intuitively, given a noisy image $\bv$, its total variation over all pixels is higher than that of the designed clean image. Therefore, to denoise an image, we aim to lower its total variation. Nonlocal functionals have been incorporated into the total variation method, allowing the notion of variation and derivative to be expressed nonlocally~\cite{Kindermann2005DeblurringAD, Gilboa2007NonlocalLI,Gilboa2008NonlocalOW}. Without some constraints, both total local and nonlocal variation methods result in image over-blurring~\cite{doi:10.1137/040616024}. 
% % On the other hand, in transformer models it is also desirable to produce smooth outputs, thus making it less susceptible to noise. 
% In this section, we establish the connection between self-attention in transformers and the total nonlocal variation denoising method. We show that self-attention in transformers implicitly lowers the total nonlocal variation of the input signals, such as images, thereby contributing to the model’s over-smoothing issue.}

We first consider the output matrix $\bU:=[\bu(1),\cdots,\bu(N)]^\top \in \RR^{N \times D}$ in self-attention as given by Eqn.~\ref{eq:attention-mat} in Section~\ref{sec:background}. Let $\Omega \subset \RR$, $x \in \Omega$, and $\bu(x):=[u_{1}(x), \dots, u_{D}(x)]^T$ be a real vector-valued function, $\bu:\Omega \rightarrow \RR^{D}$, $\bu \in L^{2}(\Omega)$. The output matrix $\bU$ in self-attention discretizes the function $\bu(x)$ on a 1-D grid. In the context of signal/image denoising, $\bU$ can be considered as the \emph{desired clean signal}, and $\bu(x)$ is its corresponding intensity function denoting the signal values at the position $x \in \Omega$. We further let the observed intensity function $\bff(x)$ denote the values of the \emph{observed noisy signal} at $x \in \Omega$, $\bff:\Omega \rightarrow \RR^{D}$, $\bff \in L^{2}(\Omega)$. For example, $\bff(x)$ can be given as
\begin{align}
\bff(x) = \bu(x) + \bn(x),
\end{align}
where $\bn$ is the additive noise. 
% A discretization of $\bv(x)$ on a 1-D grid yields the value vectors $\bv(1), \dots, \bv(N) \in \RR^{D}$, which form the value matrix $\bV:=[\bv(1),\cdots,\bv(N)]^\top \in \RR^{N \times D}$ in self-attention as defined in Eqn.~\ref{eq:attention-mat}.  
We wish to reconstruct $\bu(x)$ from $\bff(x)$. Following the variational denoising method proposed in~\cite{Gilboa2007NonlocalLI} and~\cite{Gilboa2008NonlocalOW}, the denoised image $\bu(x)$ can be obtained by minimizing the following regularized functional with respect to $\bu$:
\begin{align}
\label{eqn:energy-functional}
    E(\bu, \bff) &= J(\bu) + G(\bu,\bff) \\ \nonumber
    &= \frac{1}{2} \int_{\Omega \times \Omega} \|\bu(x) - \bu(y)\|_2^2 k(x, y)dx dy + \frac{\lambda}{2}  \int_{\Omega} \|\bu(x) - \bff(x)\|_2^2 dx.
\end{align}
Here, $J(\bu) = \frac{1}{2} \int_{\Omega \times \Omega} \|\bu(x) - \bu(y)\|_2^2 k(x, y)dxdy$ is a nonlocal functional of weighted differences. The weights $k(x, y)$ represent the affinity between signal values at positions $x$ and $y$. For example, for images, $k(x, y)$ captures the proximity between pixels $x$ and $y$ in the image. $J(\bu)$ works as a regularizer. Minimizing $J(\bu)$ promotes the smoothness of $\bu$ and penalizes high-frequency noise in the signal. Adding the convex fidelity term $G(\bu,\bff) =\frac{\lambda}{2}  \int_{\Omega} \|\bu(x) - \bff(x)\|_2^2 dx$ to the functional $J(\bu)$ allows the denoised signal $\bu(x)$ to preserve relevant information in the observed noisy signal $\bff(x)$. The regularized functional $E(\bu, \bff)$ can be considered as an energy functional.

\subsection{Self-attention as a Gradient Descent Step to Minimize the Nonlocal Functional $J$}
\label{subsec:self-attention-TV}
We show that self-attention is equivalent to
% reconstructs the desired clean signal $\bu$ from the observed noisy signal $\bv$ 
 taking a gradient descent step toward minimizing the functional $J(\bu)$ in the energy functional $E(\bu, \bff)$. We expand $J(\bu)$ as follows
\begin{align}
    J(\bu) = \frac{1}{2} \int_{\Omega \times \Omega}\sum_{j=1}^{D}(u_j(x) - u_j(y))^2 k(x, y)dxdy
\end{align}

The gradient of $J$ with respect to $\bu$ is then given by
\begin{equation}
\begin{aligned}
\label{eqn:devJu}
    \nabla_{\bu} J(\bu) = \left[\frac{\partial J}{\partial u_1}, \frac{\partial J}{\partial u_2},  \dots, \frac{\partial J}{\partial u_{D}} \right]^T.
% \label{eq:}
\end{aligned}
\end{equation}
The partial derivative ${\partial J}/{\partial u_j}$, $j = 1, 2, \dots, D$, is defined through its dot product with an arbitrary function $h_j \in L^{2}(\Omega)$ as follows
% To compute the partial derivative ${\partial J}/{\partial u_j}$, $j = 1, 2, \dots, D$, we examine how $J$ changes when we add an infinitesimally small change to $u_j$, while keeping other $u_{j \neq i}$ fixed. In particular, given $h_j$ is an arbitrary function mapping from $\Omega$ to $\mathbb{R}$, we evaluate the differential $dJ(u_j + \tau h_j) := J(\dots, u_j + \tau h_j, \dots) - J(\bu)$ as the positive scalar $\tau$ approaches 0:
\begin{align}  
    \frac{\partial J}{\partial u_j}\cdot h_j(x) &= \frac{d}{d\tau}J(u_j + \tau h_j)\bigl|_{\tau=0} \nonumber \\ 
&= \frac{1}{2} \left(\frac{d}{d\tau}  \int_{\Omega \times \Omega}(u_j(x) - u_j(y) + \tau h_j(x) - \tau h_j(y))^{2} k(x, y)dxdy\right)\biggl|_{\tau=0} \nonumber \\
&= \left(\int_{\Omega \times \Omega}(u_j(x) - u_j(y) + \tau h_j(x) - \tau h_j(y))(h_j(x) -h_j(y))k(x, y)dxdy\right)\biggl|_{\tau=0} \nonumber \\
&= \int_{\Omega \times \Omega}(u_j(x) - u_j(y))(h_j(x) -h_j(y))k(x, y)dxdy \nonumber \\
&= \int_{\Omega \times \Omega}(u_j(x) - u_j(y))h_j(x)k(x, y)dxdy - \int_{\Omega \times \Omega}(u_j(x) - u_j(y))h_j(y)k(x, y)dxdy \nonumber
% \frac{d}{d\tau} \int_{\Omega \times \Omega} \bigl(u_i(x) - u_i(y) \bigl)\bigl(h_i(x) - h_i(y) \bigl)k(x, y)dxdy.
\end{align}
Applying a change of variables $(x, y) \rightarrow (y, x)$ to the second term of the above integral, we have
\begin{align}  
\frac{\partial J}{\partial u_j} \cdot h_j(x) &= \int_{\Omega \times \Omega}(u_j(x) - u_j(y))h_j(x)k(x, y)dxdy - \int_{\Omega \times \Omega}(u_j(y) - u_j(x))h_j(x)k(y, x)dxdy \nonumber \\
&= \int_{\Omega \times \Omega}(u_j(x) - u_j(y)(k(x, y) + k(y, x))dyh_j(x)dx \nonumber
\end{align}
Thus, the Frechet derivative of J with respect to $u_j$ is given by
\begin{align}  
\label{eq:partial-dev}
\frac{\partial J}{\partial u_j} 
&= \int_{\Omega}(u_j(x) - u_j(y)(k(x, y) + k(y, x))dy. 
\end{align}
% \begin{equation}  
% \frac{d}{d\tau}J(u_i + \tau h_i)\bigl|_{\tau=0} = \int_{\Omega \times \Omega} \bigl(u_i(x) - u_i(y) \bigl)\bigl(h_i(x) - h_i(y) \bigl)k(x, y)dxdy.
% \label{eq:partial-dev}
% \end{equation}
% The detailed derivation of Eqn.~\ref{eq:partial-dev} is given in  Appendix~\ref{secapp:proof-gradient}. By splitting the integral in Eqn.~\ref{eq:partial-dev} into two terms involving $u_i(x)$ and $u_i(y)$ and by changing the position variables of the latter from $(x, y) \rightarrow (y, x)$, the partial derivatives in~\ref{eq:partial-dev} becomes\\$\int_{\Omega \times \Omega} \bigl(u_i(x) - u_i(y) \bigl)\bigl(k(x, y) + k(y, x)\bigl)h_i(x)dxdy.$ When the change in variables happens, the term $k(y, x)$ appears since, in this work, we consider asymmetric $k(y, x)$, making $k(y, x) \neq k(x, y)$. As a result, the Frechet derivative of $J$ w.r.t $u_i$ at $x$ is $\int_{\Omega} \bigl(u_i(x) - u_i(y) \bigl)\bigl(k(x, y) + k(y,x)\bigl)dy$. The derivation details of $\nabla_{\bu} J(\bu)(x)$ is presented in the Appendix~\ref{secapp:proof-gradient}.\\\\

Substituting the formula for ${\partial J}/{\partial u_j}$ in Eqn.~\ref{eq:partial-dev} into Eqn.~\ref{eqn:devJu} for $\nabla_{\bu} J(\bu)(x)$, we obtain the following gradient flow
% the gradient of $J$ w.r.t $\bu$ at $x$, 
% we derive
% \begin{equation}
% \nabla_{\bu} J(\bu)(x) = \int_{\Omega} \bigl(\bu(x) - \bu(y) \bigl)\bigl(k(x, y) + k(y,x)\bigl)dy
% \label{eq:gradient-J}
% \end{equation}
% The derivation details of $\nabla_{\bu} J(\bu)(x)$ is presented in the Appendix~\ref{sec:}. Utilizing gradient descent, to minimize $J(\bu)$, we take steps towards the reversing direction of the gradient
\begin{equation}
\begin{aligned}
    \label{eq:gradient-descent}
    \frac{d\bu(x,t)}{dt} &= -\nabla_{\bm{u}}J(\bu) = \int_{\Omega} \bigl(\bm{u}(y,t) - \bm{u}(x,t) \bigl)\bigl(k(x, y) + k(y,x)\bigl)dy,
\end{aligned}
\end{equation}
where $t$ is the time variable we introduce to capture the dynamics of $\bu$ when gradient descent is applied to minimize $J(\bu)$. Let $\bv(x):=[v_{1}(x), \dots, v_{D}(x)]^T$ be a real vector-valued function, $\bv:\Omega \rightarrow \RR^{D}$, $\bv \in L^{2}(\Omega)$. We discretize $\bv(x)$ on a 1-D grid to attain the value vectors $\bv(1), \dots, \bv(N) \in \RR^{D}$, which form the value matrix $\bV:=[\bv(1),\cdots,\bv(N)]^\top \in \RR^{N \times D}$ in self-attention as defined in Eqn.~\ref{eq:attention-mat}. We initialize $\bu$ at $t=0$ with $\bv(x)$, i.e., $\bu(x, 0) = \bv(x)$.

{\bf Self-attention is an Euler Discretization of the Gradient Flow Given in~\ref{eq:gradient-descent}.} We discretize the gradient flow in Eqn.~\ref{eq:gradient-descent} using the Euler method~\cite{euler1792institutiones} with step size $\Delta t(x) = {1}/{\int_{\Omega}\bigl(k(x, y) + k(y,x)\bigl)dy}$ and obtain the following update
\begin{align}
\label{eq:adaptive-stepsize-GD}
        \bm{u}(x, \Delta t(x)) 
        &= \bm{u}(x, 0) + \Delta t(x)\int_{\Omega} \bigl(\bm{u}(y, 0) - \bm{u}(x, 0) \bigl)\bigl(k(x, y) + k(y,x)\bigl)dy\nonumber \\
    &=\int_{\Omega}\displaystyle\frac{\bigl(k(x, y) + k(y,x)\bigl) \bm{u}(y, 0)}{\int_{\Omega}\bigl(k(x, y') + k(y',x)\bigl)dy'}dy =\int_{\Omega}\displaystyle\frac{K(x, y) \bm{v}(y)}{\int_{\Omega}K(x, y')dy'}dy.
\end{align}

% In Eqn.~\ref{eq:gradient-descent}, the change in $
% \bv$ at position $x$ is proportional to the sum of differences between $\bu(x)$ and $\bu$ at other position in the domain $\Omega$. In particular, when $\bu(x)$ is smaller or larger than the values at other positions, it will increase or decrease accordingly. This is analogous to the diffusion process in which particles or substances move from high-concentration to low-concentration regions. This suggests that the optimal solution tends to yield similar values across the domain $\Omega$. The main difference is that Eqn.~\ref{eq:gradient-descent} considers the difference at a non-local scale.\\\\

% From the above suggestion about the optimal solution $\bu$, it can be found iteratively approximated using an adaptive step size $\Delta t(x) := \frac{1}{\int_{\Omega}\bigl(k(x, y) + k(y,x)\bigl)dy}$. This adaptive stepsize tells us that when $\bu(x)$ is in proximity to its values at other positions, it indicates that the solution is converging, allowing us to take smaller steps to approach the solution. Conversely, when $\bu(x)$ is deviates from its values at other positions, larger steps can be taken to expedite progress
% \begin{equation}
% \label{eq:adaptive-stepsize-GD}
%     \begin{aligned}
%         \bm{u}^{n + 1}(x) 
%         &= \bm{u}^{n}(x) + \Delta t(x)\int_{\Omega} \bigl(\bm{u}^n(y) - \bm{u}^n(x) \bigl)\bigl(k(x, y) + k(y,x)\bigl)dy\\
%     &=\int_{\Omega}\displaystyle\frac{\bigl(k(x, y) + k(y,x)\bigl) \bm{u}^n(y)}{\int_{\Omega}\bigl(k(x, y) + k(y,x)\bigl)dy}dy.
%     \end{aligned}
% \end{equation}

Here, $K(x,y):=k(x,y) + k(y,x)$ is a symmetric kernel and $\bu(y, 0) = \bv(y)$ since $\bu$ is initialized at $t=0$ with $\bv$ as aforementioned. Let $\bk(x):=[k_{1}(x), \dots, k_{D_{qk}}(x)]^T$ be a real vector-valued function, $\bk:\Omega \rightarrow \RR^{D_{qk}}$, $\bk \in L^{2}(\Omega)$. Similar to $\bu(x)$ and $\bv(x)$, we can discretize $\bk(x)$ on a 1-D grid to attain the key vectors $\bk(1), \dots, \bk(N) \in \RR^{D_{qk}}$, which form the key matrix $\bK:=[\bk(1),\cdots,\bk(N)]^\top \in \RR^{N \times D_{qk}}$ in self-attention as defined in Eqn.~\ref{eq:attention-mat}. We choose $K(x,y) = \exp\bigl(\bk(x)^{T}\bk(y)/\sqrt{D_{qk}}\bigl)$ and rewrite Eqn.~\ref{eq:adaptive-stepsize-GD} as follows
\begin{align}
\label{eqn:sym-attn-cont}
\bm{u}(x, \Delta t(x)) &= \int_{\Omega}\displaystyle\frac{\exp\bigl(\bk(x)^{T}\bk(y)/\sqrt{D_{qk}}\bigl)}{\int_{\Omega}\exp\bigl(\bk(x)^{T}\bk(y')/\sqrt{D_{qk}}\bigl)dy'}\bv(y)dy.
\end{align}

Estimating the integrals in Eqn.~\ref{eqn:sym-attn-cont} via Monte-Carlo approximation using the key vectors $\bk(1),\dots,\bk(N) \in \RR^{D_{qk}}$ and and value vectors $\bv(1),\dots,\bv(N) \in \RR^{D}$, we obtain
\begin{align}
\label{eqn:sym-attn-disr-1}
\bm{u}(x, \Delta t(x)) &\approx \sum_{j = 1}^N\displaystyle\frac{\exp\bigl(\bk(x)^{T}\bk(j)/\sqrt{D_{qk}}\bigl)}{\sum_{j' = 1}^N\exp\bigl(\bk(x)^{T}\bk(j')/\sqrt{D_{qk}}\bigl)}\bv(j).
\end{align}

Discretizing $\bm{u}(x, \Delta t(x))$ on another 1-D grid, we attain 
\begin{align}
\label{eqn:sym-attn-disr-2}
\bm{u}(i) &\approx \sum_{j = 1}^N\displaystyle\frac{\exp\bigl(\bk(i)^{T}\bk(j)/\sqrt{D_{qk}}\bigl)}{\sum_{j' = 1}^N\exp\bigl(\bk(i)^{T}\bk(j')/\sqrt{D_{qk}}\bigl)}\bv(j) \nonumber \\
&= \sum_{j=1}^N{\rm softmax}\Big({\bk}(i)^\top{\bk}(j)/\sqrt{D_{qk}}\Big){\bv}(j),\,\,\, i=1,\dots,N.
\end{align}

Comparing Eqn.~\ref{eqn:sym-attn-disr-2} and Eqn.~\ref{eq:attention-vec}, we observe that Eqn.~\ref{eqn:sym-attn-disr-2} implement a symmetric self-attention, in which the query matrix $\bQ$ and the key matrix $\bK$ are the same, i.e. $\bW_Q = \bW_K$ where $\bW_Q$ and $\bW_K$ are the linear projections that map the input sequence $\bX$ into $\bQ$  and $\bK$ as given in Eqn.~\ref{eqn:qkv}. 

{\bf Breaking the Symmetry in Self-attention.} We apply the splitting method to compute the solution $\bu(x,t)$ given the gradient flow in Eqn.~\ref{eq:gradient-descent}. We first take a step $\Delta t_{1}(x) = 1/{\int_{\Omega}k(x, y)dy}$ using the differential $\int_{\Omega} \bigl(\bm{u}(y,t) - \bm{u}(x,t) \bigl)k(x, y)dy$
\begin{align}
\label{eq:splitting-step-1}
        \bm{u}(x, \Delta t_{1}(x)) 
        &= \bm{u}(x, 0) + \Delta t_{1}(x)\int_{\Omega} \bigl(\bm{u}(y, 0) - \bm{u}(x, 0) \bigl)k(x, y)dy \nonumber \\
        &= \int_{\Omega}\displaystyle\frac{k(x, y) \bm{u}(y, 0)}{\int_{\Omega}k(x, y')dy'}dy = \int_{\Omega}\displaystyle\frac{k(x, y) \bm{v}(y)}{\int_{\Omega}k(x, y')dy'}dy 
\end{align}
We then take the second step $\Delta t_{2}(x) = 1/{\int_{\Omega}k(y, x)dy}$ using the second differential $\int_{\Omega} \bigl(\bm{u}(y,t) - \bm{u}(x,t) \bigl)k(y, x)dy$

\begin{align}
\label{eq:splitting-step-2}
    \bm{u}(x, \Delta t_{1}(x) + \Delta t_{2}(x)) 
    &= \bm{u}(x, \Delta t_{1}(x)) + \Delta t_{2}(x)\int_{\Omega} \bigl(\bm{u}(y, \Delta t_{1}(x)) - \bm{u}(x, \Delta t_{1}(x)) \bigl)k(y, x)dy \nonumber \\
    &= \int_{\Omega}\frac{k(y, x)\bm{u}(y, \Delta t_{1}(x))}{\int_{\Omega}k(y', x)dy'}dy
\end{align}
% This symmetry of the attention scores is desirable in some image processing tasks due to the symmetric similarities between pixels, but can be relaxed for other tasks. To break the symmetry of attention scores in Eqn.~\ref{eqn:sym-attn-disr-2}, we replace the key vectors $\bk(i)$ by the query vectors $\bq(i)$, $i=1,\dots,N$, to obtain the exact formula of self-attention given by Eqn.~\ref{eq:attention-vec}. 

The following theorem summarizes our results:

% Given independent functions $\bq$ and $\bk: \Omega \rightarrow \RR^D$, by formalizing $k(x,y):= {\rm exp}\bigl({\bq(x)^T\bk(y)/\sqrt{D}}\bigl)$, and via Monte-Carlo approximation, the update step in~\ref{eq:adaptive-stepsize-GD} becomes
% \begin{equation}
% \label{eq:sym-attn-update}
% \bu^{n + 1}_i \approx \sum_{j = 1}^N \displaystyle \frac{ {\rm exp}\bigl(\bq_i^T\bk_{j}/\sqrt{D}\bigl) + {\rm exp}\bigl(\bq_j^T\bk_{i}/\sqrt{D}\bigl)}{\sum_{j = 1}^N {\rm exp}\bigl(\bq_i^T\bk_{j}/\sqrt{D}\bigl) + {\rm exp}\bigl(\bq_j^T\bk_{i}/\sqrt{D}\bigl)} \bu^n_j
% \end{equation}
% Notice that $k(x, y) + k(y, x)$ is symmetric. We also consider relaxing this symmetry by directly formulating $k(x, y) + k(y, x) := {\rm exp}\bigl({\bq(x)^T\bk(y)/\sqrt{D}}\bigl)$, we derive the softmax attention
% \begin{equation}
% \begin{aligned}
%     \bm{u}^{n + 1}_i &\approx \displaystyle \frac{\sum_{j = 1}^N {\rm exp}\bigl(\bq_i^T\bk_{j}/\sqrt{D}\bigl)\bm{u}_j^n}{\sum_{j = 1}^N{\rm exp}\bigl(\bq_i^T\bk_{j}/\sqrt{D}\bigl)}= \sum_{j = 1}^{N} {\rm softmax}\bigl(\bq_i^T\bk_{j}/\sqrt{D}\bigl)\bm{u}_j^n.
% \end{aligned}
% \end{equation}
% % where we denotes $a(x,y) := \displaystyle\frac{k(x, y) + k(y,x)}{\int_{\Omega}\bigl(k(x, y) + k(y,x)\bigl)dy}$.
\begin{theorem}[Self-attention as a Gradient Descent Step to Minimize a Nonlocal Functional]
Given the nonlocal functional $J(\bu) = \frac{1}{2} \int_{\Omega \times \Omega} \|\bu(x) - \bu(y)\|_2^2 k(x, y)dxdy$ of a vector-valued function $\bu: \Omega \to \mathbb{R}^{D}$, $\bu \in L^{2}(\Omega)$, and let $K(x,y):=k(x,y) + k(y,x) = \exp\bigl(\bk(x)^{T}\bk(y)/\sqrt{D_{qk}}\bigl)$, where $\bk:\Omega \rightarrow \RR^{D_{qk}}$, $\bk \in L^{2}(\Omega)$. Then, taking a gradient descent step on $\bu$ at time $t=0$, where $\bu(x,0)=\bv(x)$, with an adaptive step size $\Delta t(x):= \displaystyle \frac{1}{\int_{\Omega}\bigl(k(x, y) + k(y,x)\bigl)dy}$ to minimize $J$ is equivalent to updating $\bu$ via a symmetric self-attention 
\begin{align}
\bm{u}(x, \Delta t(x)) = \sum_{j=1}^N{\rm softmax}\Big({\bk}(x)^\top{\bk}(j)/\sqrt{D_{qk}}\Big){\bv}(j), \nonumber
\end{align}
which results in
\begin{align}
\label{eqn:thm-sym-attn}
\bm{u}(i) = \sum_{j=1}^N{\rm softmax}\Big({\bk}(i)^\top{\bk}(j)/\sqrt{D_{qk}}\Big){\bv}(j),\,\,\, i=1,\dots,N.
\end{align}
Here, $\bu(n)$, $\bv(n)$, and $\bu(n)$, $n=1,\dots,N$, are the key, value, and output vectors in self-attention, respectively. Breaking the symmetry of the attention scores by replacing $\bk(i)$ with $\bq(i)$, $i=1,\dots,N$, in Eqn.~\ref{eqn:thm-sym-attn}, we obtain the exact formula of self-attention
\begin{align}
\label{eqn:thm-asym-attn}
\bm{u}(i) = \sum_{j=1}^N{\rm softmax}\Big({\bq}(i)^\top{\bk}(j)/\sqrt{D_{qk}}\Big){\bv}(j),\,\,\, i=1,\dots,N. \nonumber
\end{align}

\begin{remark}
In Eqn.~\ref{eq:gradient-descent}, the change in $\bu$ at position $x$ is proportional to the sum of differences between $\bu(x)$ and $\bu$ at other position in the domain $\Omega$. In particular, when $\bu(x)$ is smaller or larger than the values at other positions, it will increase or decrease, respectively. This is analogous to a diffusion process in which particles or substances move from high-concentration to low-concentration regions. It has been proved that a diffusion process converges to a saturating state in which the concentrations at all positions are the same. This suggests that $\bu(x)$ tends to suffer from the over-smoothing issue.
% the optimal solution tends to yield similar values across the domain $\Omega$. The main difference is that Eqn.~\ref{eq:gradient-descent} considers the difference at a non-local scale.
\end{remark}


% and choosing a positive similarity function $k(x,y):= {\rm exp}\bigl({\bq(x)^T\bk(y)/\sqrt{D}}\bigl)$, via Monte-Carlo approximation, applying the following \textbf{Symmetricity Attention (Sym-Attention)}:
% \begin{equation}
% \label{eq:sym-attn-theorem}
%     \bu^{n + 1}_i = \displaystyle \frac{\sum_{j = 1}^N {\rm exp}\bigl(\bq_i^T\bk_{j}/\sqrt{D}\bigl) + {\rm exp}\bigl(\bq_j^T\bk_{i}/\sqrt{D}\bigl) \bu^n_j}{\sum_{j = 1}^N   \bigl(\bq_i^T\bk_{j}/\sqrt{D}\bigl) + {\rm exp}\bigl(\bq_j^T\bk_{i}/\sqrt{D}\bigl)}.
% \end{equation}
% lowers the energy $J(\bu)$ in~\ref{eq:engergy-function}\\
% When the symmetry of $k(x, y) + k(y, x)$ is relaxed, the term can be directly formulated as ${\rm exp}\bigl({\bq(x)^T\bk(y)/\sqrt{D}}\bigl)$,
% % $a(x,y) := \displaystyle\frac{k(x, y) + k(y,x)}{\int_{\Omega}\bigl(k(x, y) + k(y,x)\bigl)dy} = \displaystyle\frac{{\rm exp}\bigl({\bq(x)^T\bk(y)/\sqrt{D}}\bigl)}{\sum_{j = 1}^N {\rm exp}\bigl({\bq(x)^T\bk(y)/\sqrt{D}}\bigl)}$
% the update step becomes \textbf{softmax attention}:
% \begin{equation}
% \label{eq:softmax-attn-theorem}
% \bu^{n + 1} = \sum_{j = 1}^{N} {\rm softmax}\bigl(\bq_i^T\bk_{j}/\sqrt{D}\bigl)\bm{u}_j^n.
% \end{equation}
\end{theorem}
\subsection{Random Walk Analysis of Over-smoothing}
\label{subsec:rw-oversmooth}
The diffusion process and random walk are closely related concepts, as diffusion can be seen as a collective behavior of numerous random walks performed by individual particles or molecules. Inspired by the analogy between the dynamics of $\bu$ in Eqn~\ref{eq:gradient-descent} and a diffusion process, as well as the relationship between diffusion process and random walk, in this section, we show the connection between the evolution of $\bu$  and a random walk. By adopting a random walk perspective on graph neural network~\cite{Thorpe2022GRANDGN}, we demonstrate that $\bu(x)$ under the dynamics given in Eqn~\ref{eq:gradient-descent} suffers from over-smoothing.\\\\
Recall from the gradient flow in Eqn~\ref{eq:gradient-descent}, by using Euler method discretization, after $k$ update steps starting from the initial $\bu(x, 0) = \bv(x)$, with adaptive stepsize $\Delta t = \displaystyle {1}/{\int_{\Omega}\bigl(k(x, y) + k(y,x)\bigl)dy}$, we obtain the following 
\begin{align}
\label{eq:uk}
        \bm{u}(x, k\Delta t(x)) 
        % &= \bm{u}(x, (k - 1)\Delta t(x)) \nonumber \\
        % &+ \Delta t(x)\int_{\Omega} \bigl(\bm{u}(y, (k - 1)\Delta t(x)) - \bm{u}(x, (k - 1)\Delta t(x)) \bigl)\bigl(k(x, y) + k(y,x)\bigl)dy\nonumber \\
    &=\int_{\Omega}\displaystyle\frac{K(x, y) \bm{u}(y, (k - 1)\Delta t(x))}{\int_{\Omega}K(x, y')dy'}dy.
\end{align}
Discretizing $\bm{u}(x, k\Delta t(x))$ and using Monte-Carlo approximation for the integrals in~\ref{eq:uk} , we attain
\begin{align}
\label{eq:rwu}
\bm{u}^{(k)}(i) = \sum_{j = 1}^N\bA_{ij}\bu^{(k-1)}(j)
\end{align}
    where $\bA_{ij}$ is computed using the keys and queries as either ${\rm softmax}\Big({\bk}(i)^\top{\bk}(j)/\sqrt{D_{qk}}\Big)$ or ${\rm softmax}\Big({\bq}(i)^\top{\bk}(j)/\sqrt{D_{qk}}\Big)$.
Let $ \{\mathbf{B}^{(k)}(i)\}_{k \in K}$ be a random walk on $\{\bv(i)\}^N_{i = 1}$ as defined:
\begin{equation}
\label{eq:def-rw}
    \begin{aligned}
        \mathbf{B}^{(0)}(i) &= \bv(i) \\ 
        \mathbb{P}(\mathbf{B}^{(k + 1)}(l) = \bv(j) &| \mathbf{B}^{(k)}(l) = \bv(i)) = \bA_{ij}
    \end{aligned}
\end{equation}
where $\mathbf{B}^{(k)}(n)$ is the random value of a $k$-step walk, starts at node $n$, and $\bv(n)$ is the initial value at node $n$, respectively, for $n = 1, 2, \dots, N$. The transition probability $\bA$ is defined as above. To investigate the connection between the update process of $\bu$ and the random walk defined in~\ref{eq:def-rw}, we show that, for $i = 1, 2, \dots, N$, after $k$ update steps as in~\ref{eq:rwu}, with initial value
$\bu^{(0)}(i) = \bv(i)$,
% $\bV = [ \bv(1), \bv(2), \dots, \bv(N) ]^T$, 
$\bu(i)^{(k)}$ equals to the expected value of the $k$-step walk,  starting at node $i$:
\begin{lemma}
\label{prop:equivalent-rw-id-solution}
Let $\bu^{(k)}(i)$ defined in ~\ref{eq:rwu} and $\{\mathbf{B}^{(k)}(i)\}_{k \in K}$ is the random walk defined by~\ref{eq:def-rw}. Then 
\begin{align}
\bu^{(k)}(i) = \mathbb{E}[\mathbf{B}^{(k)}(i)].
\end{align}
\end{lemma} 
We next present the Lemma~\ref{prop:stationary-dis-rw} which is necessary to show the convergence of $\bu^{(k)}(i)$.
\begin{lemma}
\label{prop:stationary-dis-rw}
    The random walk $\mathbf{B}^{(k)}(i)$  in~\ref{eq:def-rw} with the transition matrix $\bA$ either be $\bA_{ij} = {\rm softmax}\Big({\bk}(i)^\top{\bk}(j)/\sqrt{D_{qk}}\Big)$ or $\bA_{ij} = {\rm softmax}\Big({\bq}(i)^\top{\bk}(j)/\sqrt{D_{qk}}\Big)$, has a unique stationary distribution $\pmb{\pi} = [\pi_1, \pi_2, \dots, \pi_N]$ such that $\pi_i := P(\mathbf{B}^{(k)}(j) = \bv(i))$, for $i,j = 1, 2, \dots, N$, $\sum_{i = 1}^N \pi_i = 1$, and $\pmb{\pi}^T = \pmb{\pi}^T\bA$. \\ \\
If $\bA_{ij} = {\rm softmax}\Big({\bk}(i)^\top{\bk}(j)/\sqrt{D_{qk}}\Big)$, the stationary distribution is:
\begin{align}
\pmb{\pi} = \Bigg( \frac{d_1}{\sum_{j = 1}^N d_j}, \frac{d_2}{\sum_{j = 1}^N d_j}, \dots, \frac{d_n}{\sum_{j = 1}^N d_j} \Bigg),
\end{align}
where $d_i = \sum_{j = 1}^N {\rm exp}\Big({\bk}(i)^\top{\bk}(j)/\sqrt{D_{qk}}\Big)$, ${\bk}(1), {\bk}(2), \dots, {\bk}(N)$ are the key vectos. \\ \\
In general, $\pi_i$ can be found by finding the left eigenvector of $\bA$ corresponding to the dominant eigenvalue 1.
\end{lemma}
% \begin{prop}
%     \label{prop:stationary-dis-rw}
% The stationary distribution of $\{\mathbf{B}^n_i\}_{n \in K}$ is 
% \begin{align}
% \pi = \Bigg( \frac{d_1}{\sum_{j = 1}^N d_j}, \frac{d_2}{\sum_{j = 1}^N d_j}, \dots, \frac{d_n}{\sum_{j = 1}^N d_j} \Bigg)
% \end{align}
% where $d_i = \sum_{j = 1}^N ( k_{ij} + k_{ji} )$
% \end{prop}
% Lemma~\ref{prop:stationary-dis-rw} shows that the stationary distribution of the random walk $\{\mathbf{B}^k_i\}_{k \in K}$ does not depend on the initial position $\{\bv_j(0)\}^N_{j = 1}$ for both Sym-Attention and softmax attention.
From the Lemma~\ref{prop:equivalent-rw-id-solution} and Lemma~\ref{prop:stationary-dis-rw}, we see that,
% \begin{prop}
% \label{prop:rw-convergence}
for all $i = 1, 2, \dots, N$, 
\begin{equation}
    \begin{aligned}
        \bu^{(k)}(i) = \mathbb{E}[\mathbf{B}^{(k)}(i)] = \sum_{j = 1}^N \bv(j) \mathbb{P}(\mathbf{B}^{(k - 1)}(i) = \bv(j)) \rightarrow \sum_{j = 1}^N \pi_j \bv(j) =: \bar{\bv}.
    \end{aligned}
\end{equation}
% \begin{align}
% \bv^k_i \rightarrow \Bar{\bv} := \sum_{j = 1}^N \bv^0_j \pi_j, 
% \end{align}
as $k \rightarrow \infty$.
% \end{prop}
This shows that when $k$ increases, $\bu(i)^{(k)}$ converges to a constant vector, indicating that $\bu(x)$, under the dynamic in~\ref{eq:gradient-descent}, suffers from over-smoothing.
% {\color{red}
% The nonlocal derivative of $v_j$ at $x$ w.r.t $y$ is defined as the difference value of $\bv$ at $x$ and $y$, weighted by a weighting function $k(x,y)$ follows~\cite{Gilboa2008NonlocalOW},
% \begin{equation}
% \label{eq:nonlocal-derivative}
%     \begin{aligned}
%     \partial_y v_j(x) = (v_j(y) - v_j(x))\sqrt{k(x, y)}.
%     \end{aligned}
% \end{equation}
% The $k(x,y)$ provides the sense of locality for the notion of nonlocal derivative. The derivative is smaller, or less weighted when two positions are far away. In our work, we concern with asymmetric $k(x, y)$.
% % where $k(x, y)$ is a positive weighting function. We assume that $k(x,y)$ is asymmetric.
% % Here, the discretized ($\bm{v}(1), \bm{v}(2), \dots, \bm{v}(n)$) are the token representations. 
% \\
% In the context of transformer models, the domain $\Omega$ can be discretized to $N$ discrete indices, and the discretized $\bv_i$, for $i = 1, 2, \dots, N$ can be considered as the $i$-th token representation. And Eqn.~\ref{eq:nonlocal-derivative} measures the weighted difference between two positions representations at feature $j$.\\ \\
% The sum of square of the non-local derivatives of $\bv_j$ over all positions $x \in \Omega$ with respect to all positions $y \in \Omega$, across all features $j$, represents the variation of the multi-channel signal $\bv$ over all positions:
% \begin{equation}
% \begin{aligned}
%     \label{eq:engergy-function}
%     E(\bm{v}) &=\frac{1}{2} \int_{\Omega}\int_{\Omega} \|\bm{v}(x) - \bm{v}(y)\|_2^2 k(x, y)dxdy\\
%             &= \frac{1}{2} \int_{\Omega}\int_{\Omega} \sum_j^{D_x}(v_j(x) - v_j(y))^2 k(x, y)dxdy,
% \end{aligned}    
% \end{equation}
% where $k(x,y)$ is a positive, asymmetric weighting function.
% % $E(\bm{v})$ is the sum of the square of non-local derivatives of $v_i$, for $i = 1, 2, \dots, D_v$, over all positions $x \in \Omega$. In other words, $E(\bm{v})$ represents the total variation of multichannel signal $\bv$ across all channel $i$.
% Hence, when the functional $E(\bv)$ is lower, the total nonlocal variation of the multichannel signal $\bv$ gets smaller, and the signal $\bv$ becomes smoother. 
% }
% Here we assume that $\bm{v}, \bq, \bk$ are independent vector-valued functions.
% To lower $E(\bv)$, the gradient descent method can be used. To move on, the following Lemma~\ref{prop:gradient-E}, which calculate the gradient of $E$ w.r.t $\bv$ is needed:
% \begin{lemma}
% \label{prop:gradient-E}
% Given the functional $E$ defined as in~\ref{eq:engergy-function} and the vector-valued function $\bv : \Omega \to \mathbb{R}^D_x$, the gradient of $E$ w.r.t $\bv$ at $x$ is computed as:
% \begin{equation}
% \begin{aligned}
%     \nabla_{\bm{v}}E(\bv)(x) &= \left[\frac{\partial E}{\partial v_1}, \frac{\partial E}{\partial v_2},  \dots, \frac{\partial E}{\partial v_{D_x}} \right]^T\\
%     &= \int_{\Omega} \bigl(\bv(x) - \bv(y) \bigl)\bigl(k(x, y) + k(y,x)\bigl)dy,
% \end{aligned}
% \end{equation}
% where the Gateaux-derivative of $E$ w.r.t $v_i$ at $x$ is:
% \begin{equation}
% \nonumber
%     \frac{\partial E}{\partial v_i}(x) = \int_{\Omega} \bigl(v_i(x) - v_i(y) \bigl)\bigl(k(x, y) + k(y,x)\bigl)dy
% \end{equation}
% \end{lemma}
% Lemma~\ref{prop:gradient-E} suggests that $E(\bv)$ decreases via gradient descent:
% One way to solve this system of equations is via gradient descent and by introducing a dummy variable time $t$
% \begin{equation}
% \begin{aligned}
%     \label{eq:gradient-descent}
%     \frac{d\bm{v}(x,t)}{dt} &= -\nabla_{\bm{v}}E(\bv)(x) = \int_{\Omega} \bigl(\bm{v}(y,t) - \bm{v}(x,t) \bigl)\bigl(k(x, y) + k(y,x)\bigl)dy,
% \end{aligned}
% \end{equation}
% where $t$ is a dummy introduced time variable.
% \begin{equation}
%     \label{eq:gradient-descent}
%     \frac{d\bm{h}(x,t)}{dt} = -\nabla_{\bm{h}}E = \int_{\Omega} \bigl(\bm{v}(y,t) - \bm{h}(x,t) \bigl)k(x, y) dy
% \end{equation}
% \begin{equation}
% \label{adaptive-stepsize-GD}
%     \begin{aligned}
%         \bm{h}^{n + 1}(x) &= \bm{h}^{n}(x) + \Delta t(x)\int_{\Omega} \bigl(\bm{v}(y) - \bm{h}^n(x) \bigl)k(x, y) dy\\
%         &= \bm{h}^{n}(x) + \int_{\Omega}\displaystyle\frac{k(x, y)\bm{v}(y)dy}{\int_{\Omega}k(x, y) dy} - \bm{h}^n(x) \int_{\Omega}\displaystyle\frac{k(x, y)dy}{\int_{\Omega}k(x, y) dy}\\
%         % &= \int_{\Omega}w(x, y)\bm{v}^n(y)dy
%     \end{aligned}
% \end{equation}
% The solution for the system of integro-differential equations~\ref{eq:gradient-descent} can be iteratively approximated with adaptive stepsize $\Delta t(x) := \displaystyle \frac{1}{\int_{\Omega}\bigl(k(x, y) + k(y,x)\bigl)dy}$
% \begin{equation}
% \label{eq:adaptive-stepsize-GD}
%     \begin{aligned}
%         \bm{v}^{n + 1}(x) 
%         &= \bm{v}^{n}(x) + \Delta t(x)\int_{\Omega} \bigl(\bm{v}^n(y) - \bm{v}^n(x) \bigl)\bigl(k(x, y) + k(y,x)\bigl)dy\\
%         % &= \bm{v}^{n}(x) + \int_{\Omega}\displaystyle\frac{\bigl(k(x, y) + k(y,x)\bigl)\bm{v}^n(y)dy}{\int_{\Omega}\bigl(k(x, y) + k(y,x)\bigl)dy} - \bm{v}^n(x) \int_{\Omega}\displaystyle\frac{\bigl(k(x, y) + k(y,x)\bigl)dy}{\int_{\Omega}\bigl(k(x, y) + k(y,x)\bigl)dy}\\
%         &= \int_{\Omega}a(x, y)\bm{v}^n(y)dy
%     \end{aligned}
% \end{equation}
% where we denotes $a(x,y) := \displaystyle\frac{k(x, y) + k(y,x)}{\int_{\Omega}\bigl(k(x, y) + k(y,x)\bigl)dy}$.
% \subsection{Self-attention as Total Nonlocal Variation}
% \begin{remark}
% Given a positive, asymmetric kernel $k(x, y)$, $a(x, y)$ is asymmetric ($a(x, y) \neq a(y, x)$). Its nominator $k(x, y) + k(y, x)$ is symmetric for any choice of $k(x, y)$. In this work, we consider both attention mechanisms with the symmetricity or the symmetricity relaxation in the norminator.
% % \end{remark}
% Assume that given independent functions $\bq$ and $\bk: \Omega \rightarrow \RR^D$, in the symmetricity setting, by formalizing $k(x,y):= {\rm exp}\bigl({\bq(x)^T\bk(y)/\sqrt{D}}\bigl)$, and via Monte-Carlo approximation, the update step in~\ref{eq:adaptive-stepsize-GD} becomes:
% \begin{equation}
% \label{eq:sym-attn-update}
% \bv^{n + 1}_i \approx \sum_{j = 1}^N \bA_{ij} \bv^n_j
% \end{equation}
% where 
% \begin{equation}
% \label{eq:sym-attn}
%     \bA_{ij} := \displaystyle \frac{ {\rm exp}\bigl(\bq_i^T\bk_{j}/\sqrt{D}\bigl) + {\rm exp}\bigl(\bq_j^T\bk_{i}/\sqrt{D}\bigl)}{\sum_{j = 1}^N   \bigl(\bq_i^T\bk_{j}/\sqrt{D}\bigl) + {\rm exp}\bigl(\bq_j^T\bk_{i}/\sqrt{D}\bigl)}.
% \end{equation}
% can be interpreted as the attention score between two discretized positions $(i, j)$ in $\Omega$, for $i, j = 1, 2, \dots, N$.\\ \\
% The approximation in~\ref{eq:sym-attn-update} is a variant of self-attention where the nominator of the normalized similarity score $\bA_{ij}$ in~\ref{eq:sym-attn} between token $i$-th and token $j$-th is symmetric. We name it the \textbf{\textit{Symmetric Attention (Sym-Attention)}}. Here, $q_i$, $k_j$ are interpreted as the query and key of token $i$-th and $j$-th, respectively.

% We also assume that $\bm{v}, \bq$ and $\bk$ are independent.
% There are two ways we can formalize the weighting functions. \\ \\
% In the symmetricity relaxation case, the symmetricity of $k(x, y) + k(y,x)$ can be relaxed by directly formulating:
% \begin{equation}
% \label{eq:direct_softmax}
%     \begin{aligned}
%         a(x,y):= \displaystyle\frac{{\rm exp}\bigl({\bq(x)^T\bk(y)/\sqrt{D}}\bigl)}{\int_{\Omega}{\rm exp}\bigl({\bq(x)^T\bk(y)/\sqrt{D}}\bigl)}.
%     \end{aligned}
% \end{equation}
% % $w(x,y):= \displaystyle\frac{{\rm exp}\bigl({\bq(x)^T\bk(y)/\sqrt{D}}\bigl)}{\int_{\Omega}{\rm exp}\bigl({\bq(x)^T\bk(y)/\sqrt{D}}\bigl)}$\\
% And via Monte-Carlo approximation, the update step in~\ref{eq:adaptive-stepsize-GD} becomes:
% \begin{equation}
% \begin{aligned}
%     \bm{v}^{n + 1}_i &\approx \sum_{j = 1}^N A_{ij}\bv_j^n = \displaystyle \frac{\sum_{j = 1}^N {\rm exp}\bigl(\bq_i^T\bk_{j}/\sqrt{D}\bigl)\bm{v}_j^n}{\sum_{j = 1}^N{\rm exp}\bigl(\bq_i^T\bk_{j}/\sqrt{D}\bigl)}\\ &= \sum_{j = 1}^{N} \text{softmax}\bigl(\bq_i^T\bk_{j}/\sqrt{D}\bigl)\bm{v}_j^n.
% \end{aligned}
% \end{equation}
% which is the softmax attention.
% We summarize our results in the following theorem:
% \begin{theorem}[Self-attention lowers total nonlocal variation of signal]
% Given the energy functional $E$ defined in Eqn.~\ref{eq:engergy-function} and a vector-valued function $\bv: \Omega \to \mathbb{R}^{D_v}$, and functions $\bq$ and $\bk: \Omega \rightarrow \RR^D$, by taking a gradient descent step with an adaptive step size $\Delta t(x):= \displaystyle \frac{1}{\int_{\Omega}\bigl(k(x, y) + k(y,x)\bigl)dy}$ and choosing a positive similarity function $k(x,y):= {\rm exp}\bigl({\bq(x)^T\bk(y)/\sqrt{D}}\bigl)$, via Monte-Carlo approximation, applying the following Symmetricity Attention (Sym-Attention):
% \begin{equation}
% \label{eq:sym-attn-theorem}
%     \bv^{n + 1}_i = \displaystyle \frac{\sum_{j = 1}^N {\rm exp}\bigl(\bq_i^T\bk_{j}/\sqrt{D}\bigl) + {\rm exp}\bigl(\bq_j^T\bk_{i}/\sqrt{D}\bigl) \bv^n_j}{\sum_{j = 1}^N   \bigl(\bq_i^T\bk_{j}/\sqrt{D}\bigl) + {\rm exp}\bigl(\bq_j^T\bk_{i}/\sqrt{D}\bigl)}.
% \end{equation}
% lowers the energy $E(\bv)$ and decrease the total nonlocal variation of the signal $\bv$. \\
% With the symmetricity relaxation, by directly formalizing $a(x,y)$ as in~\ref{eq:direct_softmax}
% % $a(x,y) := \displaystyle\frac{k(x, y) + k(y,x)}{\int_{\Omega}\bigl(k(x, y) + k(y,x)\bigl)dy} = \displaystyle\frac{{\rm exp}\bigl({\bq(x)^T\bk(y)/\sqrt{D}}\bigl)}{\sum_{j = 1}^N {\rm exp}\bigl({\bq(x)^T\bk(y)/\sqrt{D}}\bigl)}$
% , the update step becomes softmax attention:
% \begin{equation}
% \label{eq:softmax-attn-theorem}
% \bv^{n + 1} = \sum_{j = 1}^{N} \text{softmax}\bigl(\bq_i^T\bk_{j}/\sqrt{D}\bigl)\bm{v}_j^n.
% \end{equation}

% \end{theorem}
% where $\bq_i$ and $\bk_j$ are the $i$-th query and $j$-th key.\\ \\
% Secondly, by formulizing $k(x,y):= {\rm exp}\bigl({\bq(x)^T\bk(y)/\sqrt{D}}\bigl)$, and via MC approximation, we derive a novel self-attention mechanism:
% \begin{equation}
% \begin{aligned}
%         \bm{v}^{n + 1}_i &\approx \displaystyle \frac{\sum_{j = 1}^N \Bigl( {\rm exp}\bigl(\bq_i^T\bk_{j}/\sqrt{D}\bigl) + {\rm exp}\bigl(\bq_j^T\bk_{i}/\sqrt{D}\bigl) \Bigl)\bm{v}_i^n}{\sum_{j = 1}^N \Bigl( {\rm exp}\bigl(\bq_i^T\bk_{j}/\sqrt{D}\bigl) + {\rm exp}\bigl(\bq_j^T\bk_{i}/\sqrt{D}\bigl) \Bigl)}\\
%     % &= \sum_{j = 1}^N\text{softmax}\Bigl( {\rm exp}\bigl(\bq_i^T\bk_{j}/\sqrt{D}\bigl) + {\rm exp}\bigl(\bq_j^T\bk_{i}/\sqrt{D}\bigl) \Bigl)\bm{v}_i^n
% \end{aligned}
% \end{equation}
% \begin{remark}
% about q,k,v being indenpendent and NN approximation
\section{NeuTRENO: Mitigating the Over-smoothing in Transformers via Minimizing a Regularized Functional}
\label{sec:neutreno}
In Section~\ref{subsec:self-attention-TV}, we have shown that self-attention implicitly performs a gradient descent step to minimize the nonlocal functional $J(\bu)$ in Eqn.~\ref{eqn:energy-functional}, which results in the diffusive characteristics of $\bu$ and causes the over-smoothing phenomenon in transformers, as proved in Section~\ref{subsec:rw-oversmooth}. Fortunately, our objective is not to minimize $J(\bu)$ but the energy/regularized functional $E(\bu, \bff)$ defined by Eqn.~\ref{eqn:energy-functional}. This regularized functional consists of not only $J(\bu)$ but also the convex fidelity term $G(\bu,\bff) = \frac{\lambda}{2}  \int_{\Omega} \|\bu(x) - \bff(x)\|_2^2 dx$. This fidelity term aims to preserve the relevant information in the observed noisy signal $\bff(x)$ by penalizing solution $\bu(x)$ that deviates significantly from $\bff(x)$, thereby mitigating the effects of over-smoothing caused by minimizing $J(\bu)$.

In this section, we will derive our Neural Transformer with a Regularized Nonlocal Functional (NeuTRENO) by minimizing the regularized functional $E(\bu, \bff)$. We then provide a theoretical result to prove that NeuTRENO does not suffer from over-smoothing. Recall from Eqn.~\ref{eqn:energy-functional} that $E(\bu, \bff)$ is given by
\begin{equation}
    E(\bm{u}, \bff) = J(\bm{u}) + G(\bm{u}, \bff) = J(\bm{u}) + \frac{\lambda}{2} \int_{\Omega}\sum_{j=1}^{D}(u_j(x) - f_j(x))^2 dx  \nonumber
\end{equation}

Following a similar derivation as in Section~\ref{subsec:self-attention-TV} (see Appendix~\ref{secapp:grad-E} for the detailed derivation), we obtain the following gradient flow when minimizing $E(\bm{u}, \bff)$ using gradient descent 
\begin{equation}
    \label{eq:gradient-descent-Euv}
    \frac{d\bm{u}(x,t)}{dt} = -\nabla_{\bm{u}}E(\bu, \bff) = -\nabla_{\bm{u}}J(\bu) - \lambda \bigl(\bu(x) - \bff(x)\bigl),
\end{equation}

% Although lowering the nonlocal functional objective $J(\bu)$ contributes to the over-smoothing issue, we still want the output of transformer models to be smooth, hence robust to the noise. So to 
% address the issue of over-smoothing in transformers, a convex fidelity term  $F(\bu, \bv) = \frac{\lambda}{2} \int_{\Omega} c(x) \|\bu(x) - \bv(x)\|_2^2 dx$ is introduced to the functional $J(u)$. This term aims to preserve the relevant information of the input by penalizing solutions that deviate significantly from their initial values, thereby mitigating the effects of excessive smoothing. The positive weighting function $c(x)$ $c(x)$ should tell us that the more similar $\bv(x)$ is to the values of $\bv$ at all positions, the harder penalty it should get. In particular, we choose $c(x) :=\int_{\Omega}\big(k(x, y) + k(y,x)\big) dy $. Our objective function becomes
% % The positive weighting function $c(x)$ tells us that the more similar $u(x)$ is to the values of $u$ at all positions, the harder punishment it should get.
% % Although lowering the nonlocal functional objective~\ref{eq:engergy-function} contributes to the over-smoothing issue, we still want the output of transformer models to be smooth, hence robust to the noise. Therefore, instead of solely lessening the total nonlocal variation of the input signal, we regularized the solution by adding a data loss term to punish the solution that is too different from the input signal~\cite{Kindermann2005DeblurringAD,Gilboa2008NonlocalOW}. Given the initial function $\bm{v}^0$ and the regularizer $\lambda$, our objective is to minimize the energy
% \begin{equation}
% \label{eq:reg-TV}
%     E(\bm{u}, \bv) = J(\bm{u}) + F(\bm{u}, \bv)
%     % \frac{\lambda}{2}  \int_{\Omega}c(x) \|\bm{v}(x) - \bm{v}^0(x)\|_2^2 dx,
% \end{equation}

\begin{figure*}[!t]
\centering
\includegraphics[width=0.9\textwidth]{primal_dual_transformer/iclr_2023/pictures/skip-v.pdf}
% \vspace{-0.05in}
\vspace{-1em}
\caption{\small Our proposed NeuTRENO model adds a proportion of the difference between the values of the first and that of the current layer to the self-attention's output at each layer.
}

\label{fig:NeuTRENO-illustrat} 
%\vspace{-0.1in}
\end{figure*}
% \begin{equation}
%     \nabla_{\bm{v}} E_r(x) =  \nabla_{\bm{v}} E(x) + \lambda c(x)\bigl(\bm{v}(x) - \bm{v}^0(x)\bigl)
% \end{equation}
% \begin{equation}
%     \nabla_{\bm{h}} E_r(x) =  \nabla_{\bm{h}} E(x) + \lambda c(x)\bigl(\bm{h}(x) - \bm{h}^0(x)\bigl)
% \end{equation}
% \begin{equation}
%     \begin{aligned}
% \label{adaptive-stepsize-GD}
%         \bm{h}^{n + 1}(x) &= \bm{h}^{n}(x) + \Delta t(x)\nabla_{\bm{h}} E(x) - \Delta t(x)  \lambda c(x)\bigl(\bm{h}^{n}(x) - \bm{h}^0(x)\bigl)\\
%         % &= \int_{\Omega}w(x, y)\bm{v}^n(y)dy
%     \end{aligned}
% \end{equation}
% \begin{equation}
%     \nabla_{\bm{v}} E_r(x) =  \nabla_{\bm{v}} E(x) + \lambda c(x)\bigl(\bm{v}(x) - \bm{v}^0(x)\bigl)
% \end{equation}

{\bf NeuTRENO-attention is an Euler Discretization of the Gradient Flow Given in~\ref{eq:gradient-descent-Euv}.} 
% Let $\Delta t(x) = {2}/{\int_{\Omega}\bigl(k(x, y) + k(y,x)\bigl)dy}$.
% Applying the splitting method on the gradient flow in Eqn.~\ref{eq:gradient-descent-Euv}, we first take $\Delta t(x)/2$ step at $t=0$ using the gradient $-\nabla_{\bm{u}}J(\bu)$
% \begin{align}
% \label{eqn:split-1}
%     \bm{u}(x, \Delta t(x)/2)  &= \bm{u}(x, 0) - (\Delta t(x)/2)\nabla_{\bm{u}}J(\bu) = \int_{\Omega}\displaystyle\frac{K(x, y) \bm{v}(y)}{\int_{\Omega}K(x, y')dy'}dy.
% \end{align}
% Here, remind that $\bu(y, 0) = \bv(y)$. Next, we take another $\Delta t(x)/2$ at $t=\Delta t(x)/2$ using the gradient $- \lambda \bigl(\bu(x) - \bv(x)\bigl)$ and obtain
% \begin{align}
% \label{eqn:split-2}
%     \bm{u}(x, \Delta t(x)) = \bm{u}(x, \Delta t(x)/2) - \lambda(\Delta t(x)/2) \bigl(\bm{u}(x, \Delta t(x)/2) - \bv(x)\bigl)
% \end{align}
% Choosing $\lambda = 2\tilde{\lambda}/\Delta t(x)$ and plugging Eqn.~\ref{eqn:split-1} into Eqn.~\ref{eqn:split-2}, we attain the following update
% \begin{align}
% \label{eq:adaptive-split-GD}
%     \bm{u}(x, \Delta t(x)) &= \int_{\Omega}\displaystyle\frac{K(x, y) \bm{v}(y)}{\int_{\Omega}K(x, y')dy'}dy + \tilde{\lambda}\left(\bv(x) - \int_{\Omega}\displaystyle\frac{K(x, y) \bm{v}(y)}{\int_{\Omega}K(x, y')dy'}dy \right) \nonumber \\
%     &= (1- \tilde{\lambda})\int_{\Omega}\displaystyle\frac{K(x, y) \bm{v}(y)}{\int_{\Omega}K(x, y')dy'}dy + \tilde{\lambda}\bv(x).
% \end{align}
Following the similar derivation in Section~\ref{subsec:self-attention-TV}, we discretize the gradient flow in Eqn.~\ref{eq:gradient-descent-Euv} using the Euler method~\cite{euler1792institutiones} with step size $\Delta t(x) = {1}/{\int_{\Omega}\bigl(k(x, y) + k(y,x)\bigl)dy}$ and initializing $\bu$ at $t=0$ with $\bv(x)$, i.e., $\bu(x, 0) = \bv(x)$. Choosing $\lambda = \tilde{\lambda}/\Delta t(x)$, we obtain the following update
\begin{align}
\label{eq:neutreno-GD-1}
    \bm{u}(x, \Delta t(x))  &= \bm{u}(x, 0) - \Delta t(x)\nabla_{\bm{u}}J - \lambda\Delta t(x) \bigl(\bm{u}(x, 0) - \bff(x)\bigl) \nonumber \\
    &= \int_{\Omega}\displaystyle\frac{K(x, y) \bm{v}(y)}{\int_{\Omega}K(x, y')dy'}dy + \tilde{\lambda} \bigl(\bff(x) - \bm{v}(x)\bigl).
\end{align}
We choose the observed noisy signal $\bff(x)=\bv^{0}(x)$ where $\bv^{0}(x)$ is $\bv(x)$ at the first layer in the transformer model. The update in Eqn.~\ref{eq:neutreno-GD-1} becomes
\begin{align}
\label{eq:neutreno-GD-2}
    \bm{u}(x, \Delta t(x)) &= \int_{\Omega}\displaystyle\frac{K(x, y) \bm{v}(y)}{\int_{\Omega}K(x, y')dy'}dy + \tilde{\lambda} \bigl(\bv^{0}(x) - \bm{v}(x)\bigl).
\end{align}
Applying the Monte-Carlo method to approximate the integrals in Eqn.~\ref{eq:neutreno-GD-2}  and discretizing $\bm{u}(x, \Delta t(x))$, $\bm{v}(x)$, and $\bv^{0}(x)$ on a 1-D grid, we attain the following new formula for calculating symmetric self-attention:
\begin{align}
\label{eqn:neutreno-sym-attn}
\bm{u}(i) = \sum_{j=1}^N{\rm softmax}\Big({\bk}(i)^\top{\bk}(j)/\sqrt{D_{qk}}\Big){\bv}(j) + \tilde{\lambda}(\bv^{0}(i) - \bv(i)),\,\,\, i=1,\dots,N.
\end{align}
Its corresponding asymmetric self-attention is obtained by replacing the key vectors $\bk(i)$ with the query vectors $\bq(i)$, $i=1,\dots,N$, and given by
\begin{align}
\label{eqn:neutreno-asym-attn}
\bm{u}(i) = \sum_{j=1}^N{\rm softmax}\Big({\bq}(i)^\top{\bk}(j)/\sqrt{D_{qk}}\Big){\bv}(j) + \tilde{\lambda}(\bv^{0}(i) - \bv(i)),\,\,\, i=1,\dots,N.
\end{align}

Leveraging Eqn.~\ref{eqn:neutreno-asym-attn}, we define the Neural Transformer with a Regularized Nonlocal Functional (NeuTRENO) as follows.
\begin{definition}[Neural Transformer with a Regularized Nonlocal Functional (NeuTRENO)]
\label{def:bn-attn}
Given a set of key and value vectors $\{\bk^{\ell}(j),\bv^{\ell}(j)\}_{j=1}^{N}$ in each layer $\ell$, $\ell=1,\dots,L$, for each query vector $\bq^{\ell}(i)$, $i=1,\dots,N$, in the same layer, the self-attention unit at layer $\ell$ in a Neural Transformer with a Regularized Nonlocal Functional (NeuTRENO) computes the corresponding output vector $\bu^{\ell}(i)$ of the query $\bq^{\ell}(i)$ by the following attention formula:
\begin{align}
\label{eqn:neutreno-asym-attn-def}
\bm{u}^{\ell}(i) = \sum_{j=1}^N{\rm softmax}\Big({\bq}^{\ell}(i)^\top{\bk}^{\ell}(j)/\sqrt{D_{qk}}\Big){\bv}^{\ell}(j) + \tilde{\lambda}(\bv^{0}(i) - \bv^{\ell}(i)),\,\,\, i=1,\dots,N.
\end{align}
where $\bv^{0}(1),\dots \bv^{0}(N)\in \RR^{D}$ are the value vectors in the first layer of NeuTRENO. 
\end{definition}
Fig.~\ref{fig:NeuTRENO-illustrat} illustrates the architecture of NeuTRENO.


% With the new dynamic in~\ref{eq:neutreno-GD}, we present a novel transformer-based that copes with over-smoothing. 
% Similar to Section~\ref{subsec:self-attention-TV}, we consider both symmetricity constraint and relaxation settings. NeuTRENO is defined as follows.
% \begin{definition}
% % [Nonlocal Functional Tranformer (NeuTRENO)]
% Given the energy functional $E_r$ defined in Eqn.~\ref{eq:reg-TV} and a vector-valued function $\bv: \Omega \to \mathbb{R}^{D_v}$, initial function $\bv^0: \Omega \to \mathbb{R}^{D_v}$, the regularization coefficient $\lambda$ and functions $\bq$ and $\bk: \Omega \rightarrow \RR^D$, by taking a gradient descent step as in~\ref{eq:adaptive-update-r}, with an adaptive step size $\Delta t(x):= \displaystyle \frac{1}{\int_{\Omega}\bigl(k(x, y) + k(y,x)\bigl)dy}$ and choosing a positive similarity function $k(x,y):= {\rm exp}\bigl({\bq(x)^T\bk(y)/\sqrt{D}}\bigl)$, via Monte-Carlo approximation, the \textbf{\textit{Symmetric NeuTRENO (Sym-NeuTRENO)}} is defined as:
% \begin{equation}
% \begin{aligned}
% \label{eq:sym-NeuTRENO-theorem}
%     \bv^{n + 1}_i &= \displaystyle \frac{\sum_{j = 1}^N {\rm exp}\bigl(\bq_i^T\bk_{j}/\sqrt{D}\bigl) + {\rm exp}\bigl(\bq_j^T\bk_{i}/\sqrt{D}\bigl) \bv^n_j}{\sum_{j = 1}^N   \bigl(\bq_i^T\bk_{j}/\sqrt{D}\bigl) + {\rm exp}\bigl(\bq_j^T\bk_{i}/\sqrt{D}\bigl)} + \lambda \bigl(\bm{v}^0_i - \bm{v}^n_i\bigl).
% \end{aligned}
% \end{equation}
% % lowers the energy $E(\bv)$ and decrease the total variation of the signal $\bv$ but  \\
% With the symmetricity relaxation, by directly formalizing $a(x,y)$ as in~\ref{eq:direct_softmax}
% % $a(x,y) := \displaystyle\frac{k(x, y) + k(y,x)}{\int_{\Omega}\bigl(k(x, y) + k(y,x)\bigl)dy} = \displaystyle\frac{{\rm exp}\bigl({\bq(x)^T\bk(y)/\sqrt{D}}\bigl)}{\sum_{j = 1}^N {\rm exp}\bigl({\bq(x)^T\bk(y)/\sqrt{D}}\bigl)}$
% , the update step in~\ref{eq:adaptive-update-r} becomes \textbf{\textit{NeuTRENO)}}:
% \begin{equation}
% \label{eq:NeuTRENO-attn-theorem}
% \bv^{n + 1}_i = \sum_{j = 1}^{N} \text{softmax}\bigl(\bq_i^T\bk_{j}/\sqrt{D}\bigl)\bm{v}_j^n + \lambda \bigl(\bm{v}^0_i - \bm{v}^n_i\bigl).
% \end{equation}
% \end{definition}
% \vspace{-.3cm}
% \noindent Our NeuTRENO method is illustrated in Figure~\ref{fig:NeuTRENO-illustrat}.
\begin{prop}
\label{prop:src-term-less-oversmoothing}
The evolution of $\bu(x)$ under the dynamic in~\ref{eq:gradient-descent-Euv} does not converge to a constant vector as $k \rightarrow \infty$
\end{prop}
Proposition ~\ref{prop:src-term-less-oversmoothing} indicates that our NeuTRENO mitigates the over-smoothing issue, suggesting the benefit of our method.










    


==> primal_dual_transformer/ieee_style/math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> primal_dual_transformer/math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
% \newcommand{\figleft}{{\em (Left)}}
% \newcommand{\figcenter}{{\em (Center)}}
% \newcommand{\figright}{{\em (Right)}}
% \newcommand{\figtop}{{\em (Top)}}
% \newcommand{\figbottom}{{\em (Bottom)}}
% \newcommand{\captiona}{{\em (a)}}
% \newcommand{\captionb}{{\em (b)}}
% \newcommand{\captionc}{{\em (c)}}
% \newcommand{\captiond}{{\em (d)}}

% % Highlight a newly defined term
% \newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
% \newcommand{\train}{\mathcal{D}}
% \newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
% \newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
% \newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
% \def\tA{{\tens{A}}}
% \def\tB{{\tens{B}}}
% \def\tC{{\tens{C}}}
% \def\tD{{\tens{D}}}
% \def\tE{{\tens{E}}}
% \def\tF{{\tens{F}}}
% \def\tG{{\tens{G}}}
% \def\tH{{\tens{H}}}
% \def\tI{{\tens{I}}}
% \def\tJ{{\tens{J}}}
% \def\tK{{\tens{K}}}
% \def\tL{{\tens{L}}}
% \def\tM{{\tens{M}}}
% \def\tN{{\tens{N}}}
% \def\tO{{\tens{O}}}
% \def\tP{{\tens{P}}}
% \def\tQ{{\tens{Q}}}
% \def\tR{{\tens{R}}}
% \def\tS{{\tens{S}}}
% \def\tT{{\tens{T}}}
% \def\tU{{\tens{U}}}
% \def\tV{{\tens{V}}}
% \def\tW{{\tens{W}}}
% \def\tX{{\tens{X}}}
% \def\tY{{\tens{Y}}}
% \def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
% \newcommand{\etens}[1]{\mathsfit{#1}}
% \def\etLambda{{\etens{\Lambda}}}
% \def\etA{{\etens{A}}}
% \def\etB{{\etens{B}}}
% \def\etC{{\etens{C}}}
% \def\etD{{\etens{D}}}
% \def\etE{{\etens{E}}}
% \def\etF{{\etens{F}}}
% \def\etG{{\etens{G}}}
% \def\etH{{\etens{H}}}
% \def\etI{{\etens{I}}}
% \def\etJ{{\etens{J}}}
% \def\etK{{\etens{K}}}
% \def\etL{{\etens{L}}}
% \def\etM{{\etens{M}}}
% \def\etN{{\etens{N}}}
% \def\etO{{\etens{O}}}
% \def\etP{{\etens{P}}}
% \def\etQ{{\etens{Q}}}
% \def\etR{{\etens{R}}}
% \def\etS{{\etens{S}}}
% \def\etT{{\etens{T}}}
% \def\etU{{\etens{U}}}
% \def\etV{{\etens{V}}}
% \def\etW{{\etens{W}}}
% \def\etX{{\etens{X}}}
% \def\etY{{\etens{Y}}}
% \def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
% \newcommand{\pdata}{p_{\rm{data}}}
% % The empirical distribution defined by the training set
% \newcommand{\ptrain}{\hat{p}_{\rm{data}}}
% \newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% % The model distribution
% \newcommand{\pmodel}{p_{\rm{model}}}
% \newcommand{\Pmodel}{P_{\rm{model}}}
% \newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% % Stochastic autoencoder distributions
% \newcommand{\pencode}{p_{\rm{encoder}}}
% \newcommand{\pdecode}{p_{\rm{decoder}}}
% \newcommand{\precons}{p_{\rm{reconstruct}}}

% \newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

% \newcommand{\E}{\mathbb{E}}
% \newcommand{\Ls}{\mathcal{L}}
% \newcommand{\R}{\mathbb{R}}
% \newcommand{\emp}{\tilde{p}}
% \newcommand{\lr}{\alpha}
% \newcommand{\reg}{\lambda}
% \newcommand{\rect}{\mathrm{rectifier}}
% \newcommand{\softmax}{\mathrm{softmax}}
% \newcommand{\sigmoid}{\sigma}
% \newcommand{\softplus}{\zeta}
% \newcommand{\KL}{D_{\mathrm{KL}}}
% \newcommand{\Var}{\mathrm{Var}}
% \newcommand{\standarderror}{\mathrm{SE}}
% \newcommand{\Cov}{\mathrm{Cov}}
% % Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% % But then they seem to use $L^2$ for vectors throughout the site, and so does
% % wikipedia.
% \newcommand{\normlzero}{L^0}
% \newcommand{\normlone}{L^1}
% \newcommand{\normltwo}{L^2}
% \newcommand{\normlp}{L^p}
% \newcommand{\normmax}{L^\infty}

% \newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

% \DeclareMathOperator*{\argmax}{arg\,max}
% \DeclareMathOperator*{\argmin}{arg\,min}

% \DeclareMathOperator{\sign}{sign}
% \DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> primal_dual_transformer/preamble.tex <==
% ---------------------------------
%floats and figures
% ---------------------------------

% if you need to pass options to natbib, use, e.g.:
\PassOptionsToPackage{numbers, compress}{natbib}
\usepackage{amsmath}
% Recommended, but optional, packages for figures and better typesetting:
\usepackage{microtype}
\usepackage{graphicx}
\usepackage{subfigure}
\usepackage{hyperref}
\hypersetup{
    colorlinks=true,
    linkcolor=blue,
    filecolor=magenta,      
    urlcolor=cyan,
    citecolor=black
}
\urlstyle{same}
%\usepackage{array}
\usepackage{booktabs} % for professional tables
\usepackage{amsfonts}
\usepackage{bm}
%\usepackage{soul}
%\usepackage{lmodern}
%\usepackage{booktabs}
\usepackage{threeparttable}
%\usepackage{mathtools}
\usepackage{tablefootnote}

%\usepackage{cuted}
\usepackage{lipsum}
\usepackage{comment}

\usepackage{multirow}
%\usepackage[usenames, dvipsnames]{color}
\usepackage{amsmath}

\newcommand\xmod[1]{{\textcolor{blue}{#1}}}
\newcommand\zmod[1]{{\textcolor{red}{#1}}}


\usepackage{hyperref}

\usepackage{enumitem}

\usepackage{mathtools}
% \DeclarePairedDelimiter\ceil{\lceil}{\rceil}
% \DeclarePairedDelimiter\floor{\lfloor}{\rfloor}

\usepackage{wrapfig}

\usepackage{listings}

\usepackage[english]{babel}
%\usepackage[utf8x]{inputenc}

\usepackage{listings}
\usepackage{color}

\definecolor{mygreen}{rgb}{0,0.6,0}
\definecolor{mygray}{rgb}{0.5,0.5,0.5}
\definecolor{mymauve}{rgb}{0.58,0,0.82}

\lstset{ %
  backgroundcolor=\color{white},   % choose the background color
  basicstyle=\footnotesize,        % size of fonts used for the code
  breaklines=true,                 % automatic line breaking only at whitespace
  captionpos=b,                    % sets the caption-position to bottom
  commentstyle=\color{mygreen},    % comment style
  escapeinside={\%*}{*)},          % if you want to add LaTeX within your code
  keywordstyle=\color{blue},       % keyword style
  stringstyle=\color{mymauve},     % string literal style
}

%=======U S E R  D E F I N E D  M A C R O S=======
% ---------------------------------
% User Comments
% ---------------------------------
\usepackage{marginnote}
% \newcommand{\bibhref}[2]{#2}
\usepackage{soul} %text highlighting
\newcommand{\todohl}[1]{{[\hl{#1?}]}}
% \usepackage[disable]{todonotes}
% \usepackage{todonotes}
% \usepackage[colorinlistoftodos]{todonotes}
%takes in optional argument
% \newcommand{\tocite}[1]{%
% \textcolor{red}{[cite:\ifthenelse{\equal{#1}{}}{}{#1}?]}
% }


\newcommand{\ignore}[1]{}
\newcommand{\etal}{et al.~}

%version in control in draft mode
\newcommand{\versionString}{\textcolor{red}{draft-mode-[\today\ \currenttime]}}

% ---------------------------------
% Label utils
% ---------------------------------

% Usage:
% \figlabel{myfigure} creates \label{fig:myfigure}
% \figref{myfigure} references it
\newcommand{\figlabel}[1]{\label{fig:#1}}
% \newcommand{\figref}[1]{Fig.    \,\ref{fig:#1}}

% Usage:
% \seclabel{mysection} creates \label{sec:mysection}
% \secref{mysection} references it
\newcommand{\seclabel}[1]{\label{sec:#1}}
% \newcommand{\secref}[1]{Section\,\ref{sec:#1}}

\newcommand{\chlabel}[1]{\label{ch:#1}}
\newcommand{\chref}[1]{Chapter\,\ref{ch:#1}}

% Usage:
% \tablabel{mytable} creates \label{tab:mytable}
% \tabref{mytable} references it
\newcommand{\tablabel}[1]{\label{tab:#1}}
\newcommand{\tabref}[1]{Table~\ref{tab:#1}}

\newcommand{\tss}{\hspace*{0.66mm}}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% space tweaks 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\setlength{\abovecaptionskip}{0.5mm}
\setlength{\belowcaptionskip}{0mm} 
\setlength{\textfloatsep}{1.5mm}
\setlength{\dbltextfloatsep}{1.5mm}
%\renewcommand{\baselinestretch}{.9945}

\makeatletter
\newenvironment{mcases}[1][l]
 {\let\@ifnextchar\new@ifnextchar
  \left\lbrace
  \def\arraystretch{1.2}%
  \array{@{}l@{\quad}#1@{}}}
 {\endarray\right.}
\makeatother


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% symbol definitions for equations
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


==> rebuttal.tex <==
% % \begin{table}[!t]
% % \centering
% % \small
% % \caption{\small {\color{black}
% % \small Means and standard deviations over 5 runs with different random seeds of models trained on the Imagenet Classification task.}}
% %     \vspace{-0.5em}
% %     \color{black}
% %     \begin{center}
% %     \scalebox{0.85}{
% %     \begin{tabular}{l|cccc}
% %     \toprule
% %          Metric/Model & \it Softmax Deit  & NeuTRENO DeiT  & NeuTRENO Adaptation & DeiT+FeatScale& NeuTRENO DeiT + FeatScale \\
% %         \midrule
% %         Top-1 Acc (\%) & 72.17 $\pm$ 0.07 & 73.01 $\pm$ 0.09 &  79.97 $\pm$ 0.07 & \bf 80.68 $\pm$ 0.06\\
% %         Top-5 Acc (\%) & 91.02 $\pm$ 0.04 & 91.56 $\pm$ 0.05 & 95.05 $\pm$ 0.03 &\bf 95.30 $\pm$ 0.04\\
% %         \bottomrule
% %     \end{tabular}}
% %     \end{center}
% % \vspace{-0.15in}
% % \label{tab:imagenet-conv2D}
% % \end{table}
% % {\fontsize{20pt}

% \begin{table}[t!]
% % \begin{minipage}[t]{.5\textwidth}
% % \centering
% \small
% \begin{minipage}[t]{0.55\textwidth}
% \caption{\small 
% \small 
% Means and standard deviations over 5 runs with different random seeds of models trained on the Imagenet Classification task.}
%     \vspace{-1em}
%     \color{black}
%     \begin{center}
%     \scalebox{0.8}{
%     \begin{tabular}{l|cc}
%     \toprule
%          Model/Metric & Top-1 Acc (\%)  & Top-5 Acc (\%)  \\
%         \midrule
%         % \it Sym-DeiT  & 71.14  & 90.54 \\
%         % Sym-NeuTRENO DeiT & \bf 72.07 & \bf 91.22 \\
%         % % \vspace{0.2cm}
%         % \hline \hline 
%         \it Softmax DeiT-Tiny  &  72.17 $\pm$ 0.07&  91.02 $\pm$ 0.04\\
%         NeuTRENO DeiT-Tiny &  73.01 $\pm$ 0.09 &  91.56 $\pm$ 0.05\\
%         NeuTRENO Adaptation & 72.63 $\pm$ 0.07& 91.38 $\pm$ 0.03\\
%          DeiT-Tiny + FeatScale & 72.346 $\pm$ 0.06 & 91.22 $\pm$ 0.04\\
%         NeuTRENO DeiT-Tiny + FeatScale & \bf 73.23 $\pm$ 0.08 & \bf 91.73 $\pm$ 0.05\\
%         \midrule
%         \it Sym DeiT-Tiny  &  71.17 $\pm$ 0.08&  90.54 $\pm$ 0.06\\
%         Sym-NeuTRENO DeiT-Tiny & \bf 72.07 $\pm$ 0.06 & \bf 91.22 $\pm$ 0.05\\
%         \midrule
%         \it Softmax DeiT-Small  &  79.97 $\pm$ 0.05&  95.05 $\pm$ 0.03\\
%         DeiT-Small + FeatScale  &  79.96 $\pm$ 0.09&  95.06 $\pm$ 0.05\\
%         NeuTRENO DeiT-Small & \bf 80.68 $\pm$ 0.06 & \bf 95.30 $\pm$ 0.03\\
        
%         \bottomrule
%     \end{tabular}}
%     \end{center}
% \vspace{-0.2in}
% \end{minipage}%
% \hspace{.05\textwidth}
% \begin{minipage}[t]{.48\textwidth}
% \centering
% \small
% \caption{
% \small Means and standard deviations over 5 runs with different random seeds of models trained on the ADE20K image segmentation task.}

%     \vspace{-1em}
%     \color{black}
%     \begin{center}
%     \scalebox{0.85}{
%     \begin{tabular}{l|cc}
%     \toprule
%          Model/Metric & SS MIoU  & MS MIoU (\%)  \\
%         \midrule
%         % \it Sym-DeiT  &  35.18 & 36.00 \\
%         % Sym-NeuTRENO DeiT & \bf 35.68 & \bf 36.39 \\
%         % \hline\hline
%         \it Softmax DeiT  &  35.72 $\pm$ 0.45& 36.68 $\pm$ 0.42\\
%          % \hline  
%         NeuTRENO DeiT & \bf 37.24 $\pm$ 0.32 & \bf 38.06 $\pm$ 0.38\\
%         \midrule
%         \it Sym-DeiT  &  35.18 $\pm$ 0.27 & 36.00 $\pm$ 0.18\\
%         Sym-NeuTRENO DeiT & \bf 35.68 $\pm$ 0.28 & \bf 36.39 $\pm$ 0.26\\
%         \bottomrule
%     \end{tabular}}
%     \end{center}
% \vspace{-0.2in}


% % \begin{table}[!t]
% % \centering
% % \small
% % \caption{\small {\color{black}
% % \small Means and standard deviations over 5 runs with different random seeds of models trained on the ADE20K image segmentation task}}
% %     \vspace{-0.5em}
% %     \color{black}
% %     \begin{center}
% %     \scalebox{0.85}{
% %     \begin{tabular}{l|cc}
% %     \toprule
% %          Metric/Model & \it Pretrained Softmax Deit-Tiny  & Pretrained NeuTRENO DeiT-Tiny  \\
% %         \midrule
% %         SS MIoU & 35.72 $\pm$ 0.57 & \bf 37.24  $\pm$ 0.62  \\
% %         MS MIoU &  36.68 $\pm$ 0.42 & \bf 38.06 $\pm$  0.54 \\
% %         \bottomrule
% %     \end{tabular}}
% %     \end{center}
% % \vspace{-0.15in}
% % \label{tab:imagenet-conv2D}
% % % \end{table}
% \end{minipage}
% \end{table}
% % \vspace{0.08em}



% \begin{table}[!t]
% % \centering
% \small
% \begin{minipage}[t]{0.55\textwidth}
% \caption{\small {\color{black}
% \small Means and standard deviations over 5 runs with different random seeds of models trained on the WikiText-103 language model task.}}
%     \vspace{-0.5em}
%     \color{black}
%     \begin{center}
%     \scalebox{0.85}{
%     \begin{tabular}{l|cc}
%     \toprule
%          Metric/Model & \it Softmax Transformer  & NeuTRENO \\
%         \midrule
%         Valid PPL & 33.15 $\pm$ 0.07 & \bf 32.60 $\pm$ 0.08  \\
%         Test PPL &  34.29 $\pm$ 0.09& \bf 33.70 $\pm$  0.07 \\
%         \bottomrule
%     \end{tabular}}
%     \end{center}
% \vspace{-0.15in}

% % \end{minipage}%
% % \hspace{.05\textwidth}
% % \begin{minipage}[t]{.48\textwidth}


% % \small
% % \caption{\small 
% % \small Means and standard deviations over 5 runs with different random seeds of models trained on the CIFAR classification task.}
% %     \vspace{-1em}
% %     \color{black}
% %     \begin{center}
% %     \scalebox{0.8}{
% %     \begin{tabular}{l|cc}
% %     \toprule
% %          Model/Metric & \it Accuracy (\%) \\
% %         \midrule
% %         \it Kernel Transformer & 75.89  \\
% %         NeuTRENO & \bf 76.75\\
% %         \bottomrule
% %     \end{tabular}}
% %     \end{center}

% % \end{minipage}%
% % \end{table}

% \begin{table}[t!]
% % \begin{minipage}[t]{.5\textwidth}
% \centering
% \small
% \caption{\small 
% \small Top-1 and Top-5 accuracy (\%) of Sym-NeuTRENO DeiT vs.\ Sym-DeiT on the ImageNet classification task. The Sym-NeuTRENO DeiT models significantly outperform the Sym-DeiT in terms of accuracy, indicating the benefit of NeuTRENO method.}
%     \vspace{-1em}
%     \color{black}
%     \begin{center}
%     \scalebox{0.8}{
%     \begin{tabular}{l|cc}
%     \toprule
%          Model/Metric & \it Top-1 Acc (\%)  & Top-5 Acc (\%)  \\
%         \midrule
%         \it Sym-DeiT  & 71.14  & 90.54 \\
%         Sym-NeuTRENO DeiT & \bf 72.07 & \bf 91.22 \\
%         \bottomrule
%     \end{tabular}}
%     \end{center}
%  \vspace{-0.1in}
% \end{table}

% \begin{table}[t!]
% % \begin{minipage}[t]{.5\textwidth}
% \centering
% % \small
% \caption{\small  
%  Evaluation of NeuTRENO DeiT-Tiny vs. Softmax DeiT-Tiny on the ImageNet-C (mean corruption error mCE), Imagenet-A (Accuracy), and Imagenet-R (Accuracy) datasets.}
%     \vspace{-1em}
%     \color{black}
%     \begin{center}
%     \scalebox{0.8}{
%     \begin{tabular}{l|ccc}
%     \toprule
%          Model/Dataset (Metric) &  Imagenet-C (mCE)  & Imagenet-A (Accuracy \%) & Imagenet-R (Accuracy \%) \\
%         \midrule
% %         \it Softmax DeiT-Tiny  & 71.6  &  6.9  & 32.83\\
% %         NeuTRENO-DeiT-Tiny & \bf 70.1 & \bf 8.2 & \bf 33.82\\
% %         \bottomrule
% %     \end{tabular}}
% %     \end{center}
% % \vspace{-0.1in}
% % \end{table}
% % \vspace{0.08em}

% % \begin{table}[t!]
% % % \begin{minipage}[t]{.5\textwidth}
% % \centering
% % % \small
% % \caption{\small 
% %  Ablation study of different values hyperparameter $\tilde{\lambda}$ of NeuTRENO DeiT-Tiny on the ADE20K Image Segmentation task.}
% %     \vspace{-1.em}
% %     \color{black}
% %     \begin{center}
% %     \scalebox{0.85}{
% %     \begin{tabular}{l|ccccccccccc}
% %     \toprule
% %          Metric/Model & \it Pretrained Softmax &  $\tilde{\lambda} = 0.1$ &  $\tilde{\lambda} = 0.2$ &  $\tilde{\lambda} = 0.4$ &  $\tilde{\lambda} = 0.5$ &  $\tilde{\lambda} = 0.6$ &  $\tilde{\lambda} = 0.8$ &  $\tilde{\lambda} = 1.0$ &  $\tilde{\lambda} = 2.0$ \\
% %         \midrule
% %         SS MIoU & 35.72  & 34.94 & 35.60& \bf 37.54 & 37.38 & 37.24 & 36.71 &36.37 &26.25\\
% %         MS MIoU &  36.68  & 35.53 & 36.45& \bf 38.62 & 38.22 & 38.06 & 37.82 & 37.26 &27.2\\
% %         \bottomrule
% %     \end{tabular}}
% %     \end{center}
% % \vspace{-0.15in}
% % \end{table}

% % \begin{figure*}[t!]
% % \centering
% % \includegraphics[width=1.1\textwidth]{primal_dual_transformer/iclr_2023/pictures/cosine_bert.pdf}
% % \vspace{-0.05in}
% % \caption{\small The average cosine similarity between token representations of 12-layer trained (Left) and  randomly-initialized (Middle) BERT-base and NeuTRENO BERT-base on the SQuAD question answering task. We also plot the same cosine similarity scores for the trained SimCSE and NeuTRENO SimCSE models (Right) on the STS-12 semantic textual similarity task. Here, 1000 and 500 data are randomly sampled for the analysis on the SQuAD and STS-12 datasets, respectively. 
% % }
% % \end{figure*}

% % }

% % \begin{table}[!t]
% % \centering
% % \small
% % \caption{\small {\color{black}
% % \small Means and standard deviations over 5 runs with different random seeds of models trained on the Imagenet Classification task.}}
% %     \vspace{-0.5em}
% %     \color{black}
% %     \begin{center}
% %     \scalebox{0.85}{
% %     \begin{tabular}{l|cccc}
% %     \toprule
% %          Metric/Model & \it Softmax Deit  & NeuTRENO DeiT  & NeuTRENO Adaptation & DeiT+FeatScale& NeuTRENO DeiT + FeatScale \\
% %         \midrule
% %         Top-1 Acc (\%) & 72.17 $\pm$ 0.07 & 73.01 $\pm$ 0.09 &  79.97 $\pm$ 0.07 & \bf 80.68 $\pm$ 0.06\\
% %         Top-5 Acc (\%) & 91.02 $\pm$ 0.04 & 91.56 $\pm$ 0.05 & 95.05 $\pm$ 0.03 &\bf 95.30 $\pm$ 0.04\\
% %         \bottomrule
% %     \end{tabular}}
% %     \end{center}
% % \vspace{-0.15in}
% % \label{tab:imagenet-conv2D}
% % \end{table}

% \begin{table}[t!]
% % \begin{minipage}[t]{.5\textwidth}
% % \centering
% % \small
% % \begin{minipage}[t]{0.5\textwidth}
% \vspace{-0.in}
% \caption{
% % \small 
% % \small 
% Means and standard deviations over 5 runs with different random seeds of models trained on the Imagenet Classification task.}
%     \vspace{-0.15in}
    
%     \color{black}
%     \begin{center}
%     \scalebox{1.}{
%     \begin{tabular}{l|cc}
%     \toprule
%          Model/Metric & Top-1 Acc (\%)  & Top-5 Acc (\%)  \\
%         \midrule
%         % \it Sym-DeiT  & 71.14  & 90.54 \\
%         % Sym-NeuTRENO DeiT & \bf 72.07 & \bf 91.22 \\
%         % % \vspace{0.2cm}
%         % \hline \hline 
%         \it Softmax DeiT  &  72.17 $\pm$ 0.07&  91.02 $\pm$ 0.04\\
%         NeuTRENO-DeiT &  73.01 $\pm$ 0.09 &  91.56 $\pm$ 0.05\\
%         NeuTRENO Adaptation & 72.63 $\pm$ 0.07& 91.38 $\pm$ 0.03\\
%          DeiT + FeatScale & 72.346 $\pm$ 0.06 & 91.22 $\pm$ 0.04\\
%         NeuTRENO DeiT + FeatScale & \bf 73.23 $\pm$ 0.08 & \bf 91.73 $\pm$ 0.05\\
%         \bottomrule
%     \end{tabular}}
%     \end{center}
% % \label{tab:imagenet}
% \vspace{-0.08in}
% \end{table}

% \begin{table}[!t]
% \centering
% % \small
% \caption{
% % \small {\color{black}
% % \small 
% Means and standard deviations over 5 runs with different random seeds of softmax DeiT and NeuTRENO DeiT trained on the ADE20K image segmentation task}
% \vspace{-0.15in}
%     % \vspace{-0.5em}
%     \color{black}
%     \begin{center}
%     \scalebox{1.}{
%     \begin{tabular}{l|cc}
%     \toprule
%          Metric/Model & \it  Softmax Deit  &  NeuTRENO DeiT  \\
%         \midrule
%         SS MIoU & 35.72 $\pm$ 0.57 & \bf 37.24  $\pm$ 0.62  \\
%         MS MIoU &  36.68 $\pm$ 0.42 & \bf 38.06 $\pm$  0.54 \\
%         \bottomrule
%     \end{tabular}}
%     \end{center}
% \vspace{-0.07in}
% % \label{tab:imagenet-conv2D}
% % \end{table}
% % \end{minipage}
% \end{table}
% % \vspace{0.08em}



% \begin{table}[!t]
% \centering
% % \small
% \caption{
% % \small 
% {\color{black}
% % \small 
% Means and standard deviations over 5 runs with different random seeds of softmax transformer and NeuTRENO trained on the WikiText-103 language model task.}}
%     \vspace{-0.15in}
%     \color{black}
%     \begin{center}
%     \scalebox{1.}{
%     \begin{tabular}{l|cc}
%     \toprule
%          Metric/Model & \it Softmax Transformer  & NeuTRENO \\
%         \midrule
%         Valid PPL & 33.15 $\pm$ 0.07 & \bf 32.60 $\pm$ 0.08  \\
%         Test PPL &  34.29 $\pm$ 0.09& \bf 33.70 $\pm$  0.07 \\
%         \bottomrule
%     \end{tabular}}
%     \end{center}
% \vspace{-0.07in}
% % \label{tab:imagenet-conv2D}
% \end{table}

% \begin{table}[t!]
% % \begin{minipage}[t]{.5\textwidth}
% \centering
% % \small
% \caption{
% % \small 
% % \small 
%  Evaluation of NeuTRENO DeiT-Tiny vs. Softmax DeiT-Tiny on the ImageNet-C (mean corruption error mCE), Imagenet-A (Accuracy), and Imagenet-R (Accuracy) datasets.}
%     \vspace{-0.25in}
%     % \hspace{-0.52in}
%     \color{black}
%     \begin{center}
%     \scalebox{1.}{
%     \begin{tabular}{l|ccc}
%     \toprule
%          Model/Dataset (Metric) &  Imagenet-C (mCE)  & Imagenet-A (Accuracy \%) & Imagenet-R (Accuracy \%) \\
%         \midrule
%         \it Softmax DeiT-Tiny  & 71.6  &  6.9  & 32.83\\
%         NeuTRENO-DeiT-Tiny & \bf 70.1 & \bf 8.2 & \bf 33.82\\
%         \bottomrule
%     \end{tabular}}
%     \end{center}
% \vspace{-0.07in}
% % \label{tab:imagenet}
% \end{table}
% % \vspace{0.08em}

% \begin{table}[t!]
% % \begin{minipage}[t]{.5\textwidth}
% % \centering
% % \small
% \caption{
% % \small 
%  Ablation study of different values hyperparameter $\tilde{\lambda}$ of NeuTRENO DeiT-Tiny on the ADE20K Image Segmentation task.}
%     \vspace{-0.07in}
%     \hspace{-0.5in}
%     \color{black}
%     % \begin{center}
%     \scalebox{1.}{
%     \begin{tabular}{l|ccccccccccc}
%     \toprule
%          Metric/Model & \it Baseline &  $\tilde{\lambda} = 0.1$ &  $\tilde{\lambda} = 0.2$ &  $\tilde{\lambda} = 0.4$ &  $\tilde{\lambda} = 0.5$ &  $\tilde{\lambda} = 0.6$ &  $\tilde{\lambda} = 0.8$ &  $\tilde{\lambda} = 1.0$ &  $\tilde{\lambda} = 2.0$ \\
%         \midrule
%         SS MIoU & 35.72  & 34.94 & 35.60& \bf 37.54 & 37.38 & 37.24 & 36.71 &36.37 &26.25\\
%         MS MIoU &  36.68  & 35.53 & 36.45& \bf 38.62 & 38.22 & 38.06 & 37.82 & 37.26 &27.2\\
%         \bottomrule
%     \end{tabular}}
%     % \end{center}
% \vspace{-0.01in}
% % \label{tab:imagenet-conv2D}
% \end{table}

% \begin{figure*}[t!]
% \label{random_bert}
% \centering
% \includegraphics[width=1.1\textwidth]{primal_dual_transformer/iclr_2023/pictures/cosine_bert.pdf}
% % \vspace{-0.05in}
% \caption{
% % \small 
% The average cosine similarity between token representations of 12-layer trained (Left) and  randomly-initialized (Middle) BERT-base and NeuTRENO BERT-base on the SQuAD question answering task. We also plot the same cosine similarity scores for the trained SimCSE and NeuTRENO SimCSE models (Right) on the STS-12 semantic textual similarity task. Here, 1000 and 500 data are randomly sampled for the analysis on the SQuAD and STS-12 datasets, respectively. 
% }
% \end{figure*}

